EAT: a simple and versatile semantic representation format for multi-purpose NLP

Semantic representations are central in many NLP tasks that require human-interpretable data. The conjunctivist framework - primarily developed by Pietroski (2005, 2018) - obtains expressive representations with only a few basic semantic types and relations systematically linked to syntactic positions. While representational simplicity is crucial for computational applications, such findings have not yet had major influence on NLP. We present the first generic semantic representation format for NLP directly based on these insights. We name the format EAT due to its basis in the Event-, Agent-, and Theme arguments in Neo-Davidsonian logical forms. It builds on the idea that similar tripartite argument relations are ubiquitous across categories, and can be constructed from grammatical structure without additional lexical information. We present a detailed exposition of EAT and how it relates to other prevalent formats used in prior work, such as Abstract Meaning Representation (AMR) and Minimal Recursion Semantics (MRS). EAT stands out in two respects: simplicity and versatility. Uniquely, EAT discards semantic metapredicates, and instead represents semantic roles entirely via positional encoding. This is made possible by limiting the number of roles to only three; a major decrease from the many dozens recognized in e.g. AMR and MRS. EAT's simplicity makes it exceptionally versatile in application. First, we show that drastically reducing semantic roles based on EAT benefits text generation from MRS in the test settings of Hajdik et al. (2019). Second, we implement the derivation of EAT from a syntactic parse, and apply this for parallel corpus generation between grammatical classes. Third, we train an encoder-decoder LSTM network to map EAT to English. Finally, we use both the encoder-decoder network and a rule-based alternative to conduct grammatical transformation from EAT-input.

==> chapters/Comparison-MRS.tex <==
\section{Comparison between MRS and EAT for text reconstruction} 
\label{sec:comparison-mrs}

In this section we empirically demonstrate that limiting the range of arguments in semantic representations along the lines specified in Sections \ref{sec:Background}--\ref{sec:EAT} can benefit \emph{text reconstruction}. As our starting point, we used the linearized MRS implementation from \citet{Hajdiketal2019}. We then modified MRS to use significantly fewer argument classes, assimilating roles as motivated by our theoretical framework (Section \ref{sec:Background}). We retained everything else in the original MRS to ensure that the differences arise only from the change in roles. Hence, here we did not implement the EAT-format as such (Section \ref{sec:EAT}), but rather a more EAT-esque variant of MRS that we call \emph{MRS-EAT}.
%We relied on \citet{Hajdiketal2019} in the choice of data, model architecture, and hyperparameters.

\subsection{Data}
We used the scripts from Hajdik et al.'s (\citeyear{Hajdiketal2019}) GitHub repository,\footnote{\url{https://github.com/shlurbee/dmrs-text-generation-naacl2019}} which also loads the training data, validation, and test data. This data is derived from the Redwoods Treebank corpus \citep{Oepenetal2002}.\footnote{\url{http://svn.delph-in.net/erg/tags/1214/tsdb/gold}} The training set size is $67313$, the validation set size $5288$, and the test set size $10201$. We note that loaded training set was smaller than the training set reported in \citet{Hajdiketal2019}, which had 72190 sentences. This is likely due to the filtering of problematic parses (e.g. parenthesis mismatches) or the exclusion of overlapping elements with the validation or test sets, both automatically conducted at the data collection and pre-processing stages of the script.
%Due to this mismatch, our results with the original MRS-format (first row of Table \ref{tab:MRS}) are not identical to those in in \citet{Hajdiketal2019}.
%We also report a wider range of textual similarity metrics, distinguishing between BLEU 1--4, and including METEOR \citep{Banerjee:Lavie2005}.

\subsection{Approach}

MRS maintains semantic compositionality while tolerating some degree of ambiguity (in e.g. quantifier scope) when disambiguation is not possible using the syntactic structure alone \citep{Copestakeetal2005}. It has been designed for typed feature-structure parsing frameworks, particularly \emph{Head-driven phrase structure grammar} (HPSG) \citep{Pollard:Sag94}.
%\citet{Lin:Xue2019} provide a detailed comparison between MRS and AMR in parsing and text generation. They account for MRSs generally higher performance on three main grounds: (i) AMR's higher degree of abstraction from surface forms, (ii) AMR's finer-grained classification of named entities, and (iii) MRS's semantic roles bearing a closer relation to syntactic roles.

\emph{Dependency MRS} (DMRS) is a graph-representation of MRS, with nodes designating word meanings and edges their semantic relations \citep{Copestake2009}.
%Compared to the original MRS, the benefit of DMRS as input for text generation is that it allows straight-forward linearization via graph-traversal (\citealt{Goodman2018}; \citeyear{Goodman2020}).
%In the remainder of this section, we talk about DMRS when using the term ``MRS''.
%Python tools for processing MRS and DMRS are included in the PyDelphin project \citep{Goodman2019}.\footnote{\url{https://github.com/delph-in/pydelphin}}
\citet{Hajdiketal2019} used DMRS linearized in the Penman format \citep{Goodman2020} for text generation via NMT, training the system to reconstruct original English sentences.
They achieved significantly better performance (33.8 vs. 75.8 BLEU-score) than AMR-based reconstruction in the same test setting \citep{Konstas2017}.
%As \citet{Hajdiketal2019} maintain, one likely reason for this improvement is that unlike AMR, (D)MRS retains grammatical information like tense.

We replicated the experiment settings of \citet{Hajdiketal2019}. The DMRS-representations contained $52$ possible semantic relation types altogether, which is why we denote it as \emph{MRS_{52}}. To shift the representation closer to EAT without changing the Penman format itself, we kept everything intact except for the role labels, which we reduced based on the theoretical discussion in Section \ref{sec:EAT}.
We call MRS with EAT-inspired reduced arguments \emph{MRS-EAT}.

MRS is \emph{hierarchical}, and all arguments (including modifiers) are dominated by their head.
Hence, modifiers in MRS-EAT require a separate \emph{M-role}.
We treated every argument that was not the A- or T-role as a modifier.
%This is because MRS is \emph{hierarchical}: each modifier is dominated by the element it modifies.
The E-role in turn is implicit, as anything dominating an A- or T-argument is automatically their E-role. Hence, the maximally reduced variant of MRS-EAT had three argument types: A, T and M. We call this variant \emph{MRS-EAT_3}.

We additionally experimented on a more grammatically sophisticated variant of MRS-EAT that had nine argument types altogether: \emph{MRS-EAT_9}. In addition to the standard A and T, MRS-EAT_9 recognized \emph{clausal} arguments A-CLAUSE and T-CLAUSE. Additionally, it separates \emph{prepositions} from other modifiers (P), and has special marking for the prepositional T-role (T-PREP). Finally, it distinguishes the left- and right-arguments of \emph{connectives} from standard A- and T-roles, and allocates them to separate roles (L-CONN and R-CONN).
Table \ref{tab:MRS-EAT-conversion} demonstrates the conversion from MRS_{52} to both variants of MRS-EAT.

\begin{table}[t]
\begin{center}
\begin{tabular}{|l|c|c|} \hline
\textbf{MRS_{52}} & \textbf{MRS-EAT_9} & \textbf{MRS-EAT_3} \\ \hline
ARG1-NEQ & A & \multirow{5}{*}{A} \\ \cline{1-2}
ARG1-H & A-CLAUSE & \\ \cline{1-2}
L-INDEX-NEQ & \multirow{3}{*}{L-CONN} & \\ \cline{1-1}
L-HNDL-HEQ & & \\ \cline{1-1}
L-HNDL-H & & \\ \hline
ARG2-NEQ (of verbs) & T & \multirow{6}{*}{T} \\ \cline{1-2}
ARG2-NEQ (of prepositions) & T-PREP & \\ \cline{1-2}
ARG2-H & T-CLAUSE & \\ \cline{1-2}
R-INDEX-NEQ & \multirow{3}{*}{R-CONN} & \\ \cline{1-1}
R-HNDL-HEQ & & \\ \cline{1-1}
R-HNDL-H & & \\ \hline
prepositions (POS-tag ``p'') & P & \multirow{2}{*}{M} \\ \cline{1-2}
rest & M & \\ \hline
\end{tabular}
\caption{Conversion from MRS to MRS-EAT.}
\label{tab:MRS-EAT-conversion}
\end{center}
\end{table}

For training the model, the script uses OpenNMT \citep{Kleinetal2017}.\footnote{\url{https://opennmt.net/}} We replicated the best-performing model architecture from \citet{Hajdiketal2019}. The initial embedding layer had 500 dimensions, and both the encoder and decoder were two-layered 800-dimensional LSTMs. Training used the negative log-likelihood loss function, dropout probability of $0.3$, and the Adam optimizer \citep{ADAM14} initialized with a $0.001$ learning rate.
We trained the model separately with each of the three input formats: MRS, MRS-EAT_9, and MRS-EAT_4. With a batch size of $50$, each model's validation accuracy stagnated or decreased after $14$ training epochs. The number of training iterations was thus identical for each model.

\subsection{Results}
\label{sec:MRS-results}

Table \ref{tab:MRS} shows the performance of the NMT models trained on MRS_{52}, MRS-EAT_{9}, and MRS-EAT_{3} on five metrics.
\emph{BLEU} \citep{Papinenietal02a} is a common metric for evaluating machine translation based on n-gram overlap between the candidate translation and the baseline.
%It has been shown to correlate with human judgement, especially on larger corpora \citep{Papinenietal02b, Coughlin2003}.
We distinguish between n-grams of length $1-4$.
\emph{METEOR} \citep{Banerjee:Lavie2005} is also based on n-gram overlap, but additionally considers paraphrases and WordNet synonyms \citep{Wordnet95}.
For both BLEU and METEOR, we used the implementations from \textit{nlg-eval}.\footnote{\url{https://github.com/Maluuba/nlg-eval}}
Finally, we also measured the ratio of \emph{exact matches}, i.e. generated texts that were identical with the original. We lowercased both original and generated texts.

\begin{table}[t]
\begin{center}
\begin{tabular}{|c|c|c|c|c|c|c|}
\hline
\textbf{Technique} & \textbf{BLEU-1} & \textbf{BLEU-2} & \textbf{BLEU-3} & \textbf{BLEU-4} & \textbf{METEOR} & \textbf{Exact match} \\ \hline
MRS & $83.28$ & $75.82$ & $69.66$ & $64.22$ & $47.60$ & $20.2\%$ \\
MRS-EAT_9 & $\mathbf{83.66}$ & $\mathbf{76.23}$ & $\mathbf{70.13}$ & $\mathbf{64.76}$ & $\mathbf{48.05}$ & $\mathbf{23.8\%}$ \\
MRS-EAT_3 & $81.40$ & $73.30$ & $66.75$ & $61.06$ & $45.96$ & $17.9\%$ \\ \hline
\end{tabular}
\caption{Comparison between the original MRS and two variants of MRS-EAT in text generation performance.}
\label{tab:MRS}
\end{center}
\end{table}

All techniques reached similar scores, differences never exceeding four points in BLEU or METEOR. Even though MRS-EAT_3 had reduced the number of arguments to a small fraction of the original MRS_{52} ($5.8\%$), performance reduction remained relatively minor: BLEU reduced by $1.88-3.16$, METEOR by $1.64$, and exact matched by $2.3\%$. More surprisingly, MRS-EAT_9 \emph{increased} the performance from MRS_{52} in all metrics: BLEU by $0.38-0.54$, METEOR by $0.45$, and exact matches by $3.6\%$.

The results illustrate that appropriate reduction of argument roles in MRS can not only significantly simplify the representation, but \emph{improve} text reconstruction.
A likely reason for this is the increased generalizability of the model, which can reduce overfitting to very specific training data features.
When reducing roles in this way, it is crucial that they are appropriately selected to optimize expressivity (somewhat analogically to dimensionality reduction).
The success of MRS-EAT_{9} indicates that its selection of roles is at least a beneficial reduction, if not even optimal.
Furthermore, even though MRS-EAT_{3} had lower performance than MRS_{52}, the differences were relatively minor in comparison to the scale of the role reduction.
We take this to indicate that optimizing semantic roles deserves more focus in future work on semantic representation.
